Nonadiabatic molecular dynamics simulation with external field

Nonadiabatic molecular dynamics simulations with classical path approximation (CPA-NAMD) cannot simulate the carrier dynamics under an external field. We develop CPA-NAMD-extF, a first-principles density-matrix framework for calculating field-driven electronic responses along precomputed finite-temperature ionic trajectories. The method combines explicit external-field coupling with self-consistent updates of electronic density while retaining the computational efficiency of the classical-path approximation. Benchmarks against regular TDDFT methods show close agreement for time-dependent dipoles, finite-field currents, and linear optical responses. Applications to the linear absorption spectrum of crystalline and amorphous SiO$_2$ demonstrate its capability to large and structurally complex systems. This method is also applied to the 2D hybrid perovskite $(\mathrm{BA})_2\mathrm{CsPb}_2\mathrm{Br}_7$. Finite-temperature calculations show that the second-order opto-current response is strongly affected by structural fluctuations. Real-space DC current density further reveals pronounced Br-centered vortex currents, and its microscopic origin is investigated.

==> shared/main-crossrefs.tex <==
% Stable labels used by the separately compiled SI to reference the main text.
\newlabel{fig:real-space-current}{{4}{}{}{}{}}

